Near-light Photometric Stereo with Symmetric Lights

This paper describes a linear solution method for near-light photometric stereo by exploiting symmetric light source arrangements. Unlike conventional non-convex optimization approaches, by arranging multiple sets of symmetric nearby light source pairs, our method derives a closed-form solution for surface normal and depth without requiring initialization. In addition, our method works as long as the light sources are symmetrically distributed about an arbitrary point even when the entire spatial offset is uncalibrated. Experiments showcase the accuracy of shape recovery accuracy of our method, achieving comparable results to the state-of-the-art calibrated near-light photometric stereo method while significantly reducing requirements of careful depth initialization and light calibration.

==> mlpreamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% mlpreamble.tex
% Matsushita Lab LaTex preamble
%
% Originally created: Aug 6th, 2019
% Version: 0.1
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\RequirePackage{booktabs}

% Reference commands
\newcommand{\Tref}[1]{Table~\ref{#1}}
\newcommand{\eref}[1]{Eq.~\eqref{#1}}
\newcommand{\Eref}[1]{Equation~\eqref{#1}}
\newcommand{\fref}[1]{Fig.~\ref{#1}}
\newcommand{\Fref}[1]{Figure~\ref{#1}}
\newcommand{\sref}[1]{Sec.~\ref{#1}}
\newcommand{\Sref}[1]{Section~\ref{#1}}


% Comment commands
\usepackage{xcolor}
\newcounter{todos}
\AtEndDocument{\ifnum\value{todos}>0 \PackageWarning{TODOS}{There are \arabic{todos} todos left in this paper! Fix them before submitting the paper!} \fi}
\newcommand{\ym}[1]{\protect\stepcounter{todos}\textcolor{magenta}{{[YM: #1]}}}
\newcommand{\fo}[1]{\protect\stepcounter{todos}\textcolor{cyan}{{[FO: #1]}}}
\newcommand{\hs}[1]{\protect\stepcounter{todos}\textcolor{teal}{{[HS: #1]}}}
\newcommand{\lm}[1]{\protect\stepcounter{todos}\textcolor{brown}{{[LM: #1]}}}
\newcommand{\heng}[1]{\protect\stepcounter{todos}\textcolor{blue}{{[HG: #1]}}}
\newcommand{\todo}[1]{\protect\stepcounter{todos}\textcolor{red}{{[TODO: #1]}}}

\newcommand{\delete}[1]{{\textcolor[rgb]{0.6,0,0}{\{#1\}}}}
\newcommand{\add}[1]{{\textcolor[rgb]{0,0.6,0}{{#1}}}} 
\newcommand{\change}[2]{\delete{#1} \add{#2}}
\newcommand{\note}[1]{{\textcolor[rgb]{0,0.6,0.6}{\textbf{Note:} #1}}}

% Operators, basic concepts
\newcommand{\argmax}{\mathop{\mathrm{argmax}}\limits}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}\limits}
\newcommand{\rank}[1]{\mathsf{rank}\left(#1\right)}		% matrix rank
\newcommand{\norm}[1]{\left\|#1\right\|}				% vector/matrix norm
\newcommand{\Span}[1]{\mathsf{span}\left\{#1\right\}}	% space spanned by vectors
\renewcommand{\dim}[1]{\mathsf{dim}\left(#1\right)}		% dimension of a space
\newcommand{\ran}[1]{\mathsf{ran}\left(#1\right)}		% range of a matrix
\newcommand{\Null}[1]{\mathsf{null}\left(#1\right)}		% null space of a matrix
\newcommand{\doubleR}{\mathbb{R}}
\newcommand{\doubleS}{\mathbb{S}}

% Vector, matrix 
\newcommand{\V}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\trace}{\ensuremath{\mathrm{tr}}}
\newcommand*{\transp}{^{\mkern-1.5mu\mathsf{T}}}
\newcommand*{\inv}{^{\mkern-1.5mu\mathsf{-1}}}

% Colors
\definecolor{lightblue}{rgb}{0.267,0.77,0.796}
\definecolor{yellow}{rgb}{0.97,0.5,0.0}
% \definecolor{pink}{rgb}{0.96,0.24,0.321}
\definecolor{pink}{rgb}{0.72,0.039,0.2}
\definecolor{orange}{rgb}{1.,0.572,0}
\definecolor{green}{rgb}{0.22,0.654,0.64}
\definecolor{purple}{rgb}{0.172,0.18,0.859}


% \newcommand{\delete}[1]{{\textcolor[rgb]{0.6,0,0}{\{#1\}}}}
% Mymacros

